Robustifying $\ell_\infty$ Adversarial Training to the Union of Perturbation Models

Classical adversarial training (AT) frameworks are designed to achieve high adversarial accuracy against a single attack type, typically $\ell_\infty$ norm-bounded perturbations. Recent extensions in AT have focused on defending against the union of multiple perturbations but this benefit is obtained at the expense of a significant (up to $10\times$) increase in training complexity over single-attack $\ell_\infty$ AT. In this work, we expand the capabilities of widely popular single-attack $\ell_\infty$ AT frameworks to provide robustness to the union of ($\ell_\infty, \ell_2, \ell_1$) perturbations while preserving their training efficiency. Our technique, referred to as Shaped Noise Augmented Processing (SNAP), exploits a well-established byproduct of single-attack AT frameworks -- the reduction in the curvature of the decision boundary of networks. SNAP prepends a given deep net with a shaped noise augmentation layer whose distribution is learned along with network parameters using any standard single-attack AT. As a result, SNAP enhances adversarial accuracy of ResNet-18 on CIFAR-10 against the union of ($\ell_\infty, \ell_2, \ell_1$) perturbations by 14%-to-20% for four state-of-the-art (SOTA) single-attack $\ell_\infty$ AT frameworks, and, for the first time, establishes a benchmark for ResNet-50 and ResNet-101 on ImageNet.

==> Suppl_Old.tex <==

\begin{appendices}

% \setcounter{tocdepth}{2}
% {\color{black}\tableofcontents}

% \newpage

\section{Robustness Stress Tests}
\label{app::StressTest}
We conduct robustness stress tests to confirm that the benefits of SNAP are sustained for a range of attack  norm-bounds, larger number of attack steps, and even for ``gradient-free'' attacks. For these experiments, we consider networks trained using TRADES and TRADES+SNAP rows in Table~2 since they achieve the highest $\mathcal{A}^{(U)}_{\text{adv}}$ among the four SOTA AT frameworks.

\subsection{Sweeping norm-bounds and number of attack steps}

We sweep the number of PGD attack steps ($K$) and norm-bounds ($\epsilon$) for all three perturbation models $(\ell_\infty,\ell_2,\ell_1)$ to confirm that the robustness gains via SNAP are achieved for a wider range of the attack norm bounds, and are sustained even after increasing attack steps. 
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\linewidth]{figures/TRADES_norm_stp_swp.pdf}
	\end{center}
	\vspace{-0.4cm}
	\caption{ResNet-18 CIFAR-10 results: Adversarial accuracy \vs norm bound $\epsilon$ for: (a) $\ell_\infty$, (b) $\ell_2$, (c) $\ell_1$ PGD-100 attack. Adversarial accuracy \vs attack steps $K$ for (d) $\ell_\infty$ ($\epsilon=0.031$), (e) $\ell_2$ ($\epsilon=0.5$), (f) $\ell_1$ ($\epsilon=12$) PGD-100 attacks.
	%with $\epsilon=(0.031,0.5,12)$, respectively.
	}
	\label{fig::SuppStepsSwp} 
	\vspace{-0.25cm}
\end{figure}



Fig.~\ref{fig::SuppStepsSwp}(a)-(c) validates the main text Table~2 conclusion that TRADES+SNAP achieves large gains ($\sim20\%$) in $\mathcal{A}^{(\ell_1)}_{\text{adv}}$ and $\mathcal{A}^{(\ell_2)}_{\text{adv}}$ with a small ($\sim4\%$) drop in $\mathcal{A}^{(\ell_\infty)}_{\text{adv}}$. Furthermore, this conclusion holds for a large range of $\epsilon$ values for all three perturbation models. Additionally, the gains in $\mathcal{A}^{(\ell_2)}_{\text{adv}}$ due to SNAP at $\epsilon=1.2$ is greater than the ones reported in Table~2 for $\epsilon=0.5$.

Now we increase the attack steps $K$ to 500 and observe the impact on adversarial accuracy against $(\ell_\infty,\ell_2,\ell_1)$ perturbation models in Fig.~\ref{fig::SuppStepsSwp}(d,e,f), respectively. In all cases, we observe hardly any change of the adversarial accuracy beyond $K=100$. Hence, as noted in the main text, we have chosen $K=100$ for all our experiments in the main text and in this supplementary. 

Recall we employ 10 random restarts as recommended by \citet{maini2019adversarial}  for \emph{all} our adversarial accuracy evaluations on CIFAR-10 data.


\subsection{Evaluating robustness against new attacks}
We evaluate adversarial accuracy against the recent DDN~\cite{rony2019decoupling} and boundary~\cite{brendel2018decision} attacks. The DDN attack was shown to be one of the SOTA gradient-based attacks, while boundary attack is one of the strongest ``gradient-free'' attacks. Of all the attacks considered in \citet{maini2019adversarial}, PGD turns out to be the strongest for $\ell_\infty$ and $\ell_1$ perturbation models. Hence, in this section, we evaluate against $\ell_2$ norm-bounded DDN  and boundary attacks. % was  

Following \citet{maini2019adversarial}, we use the FoolBox~\cite{rauber2017foolboxnative} implementation of the boundary attack, which uses 25 trials per iteration. For DDN attack, we use 100 attack steps with appropriate logit averaging for $N_0=8$ noise samples \emph{before} computing the gradient in each step (similar to our PGD attack implementations). As mentioned in the main text, it eliminates any gradient obfuscation due to the presence of noise. 
\begin{table}[t]
	\centering
	\resizebox{0.7\columnwidth}{!}{
	\begin{tabular}{|c|>{\centering\arraybackslash}p{3cm}|>{\centering\arraybackslash}p{3cm}| } %
		\hline
		 &  {\makecell{TRADES} } & {\textbf{TRADES+SNAP }} \\ 
		\hline
		{\makecell{Natural Accuracy}}  & \textbf{82.1} & {80.9}    \\
    	\hline
		 \makecell{DDN~{\small\cite{rony2019decoupling}} {\small ($\epsilon=0.5$)} }  & {59.7}  & \textbf{65.8}  \\
		 \hline
		 \makecell{Boundary~{\small\cite{brendel2018decision}} {\small ($\epsilon=0.5$)} }  & {63.5}  & \textbf{67.0}  \\
		 \hline
		 \makecell{Square~{\small\cite{andriushchenko2020square}} {\small ($\epsilon=0.5$)} }  & {68.2}  & \textbf{72.7}  \\
		 \hline
	\end{tabular}}
	\caption{ResNet-18 CIFAR-10 results showing natural accuracy (\%) and adversarial accuracy (\%) against $\ell_2$ norm bounded DDN attack~\cite{rony2019decoupling}, boundary attack~\cite{brendel2018decision}, and Square~\cite{andriushchenko2020square} for TRADES and TRADES+SNAP networks from Table~2 in the main text.} %
	\label{tab::MoreAttck}
\end{table}

Table~\ref{tab::MoreAttck} shows that SNAP improves adversarial accuracy against the DDN attack by $\sim 6\%$. This is similar to improvements seen against $\ell_2$-PGD attack in Table~2 in the main text. Similarly, TRADES+SNAP achieves $3.5\%$ higher adversarial accuracy than TRADES against the boundary attack. 


\section{Additional Results}

\subsection{Comparison with Randomized Smoothing (RS)}
\label{app::RandSmooth}
In this subsection, we compare with two SOTA randomized smoothing (RS) works, namely, RandSmooth~\cite{cohen2019certified}, and  SmoothAdv~\cite{salman2019provably}. They employ isotropic Gaussian noise. In Fig.~\ref{fig::RSComp}(a), we find that PGD+SNAP achieves better $\mathcal{A}_\text{nat}$ \vs $\mathcal{A}^{(U)}_\text{adv}$ trade-off compared to both RandSmooth~\cite{cohen2019certified}, and  SmoothAdv~\cite{salman2019provably}. Specifically, note that SmoothAdv~\cite{salman2019provably} can also be viewed as isotropic Gaussian augmentation of $\ell_2$-PGD AT. Importantly, PGD+SNAP achieves 12\% higher $\mathcal{A}^{(U)}_\text{adv}$ for same $\mathcal{A}_\text{nat}$. This demonstrates the efficacy of shaped noise in enhancing the robustness to the union of $(\ell_\infty,\ell_2,\ell_1)$ perturbations. 

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\linewidth]{figures/RandSmooth_comp.pdf}
	\end{center}
	\vspace{-0.4cm}
	\caption{ResNet-18 CIFAR-10 results: $\mathcal{A}_\text{nat}$ \vs $\mathcal{A}^{(U)}_\text{adv}$ for RandSmooth~\cite{cohen2019certified},  SmoothAdv~\cite{salman2019provably}, and PGD+SNAP (b) $\mathcal{A}_\text{nat}$ \vs $\mathcal{A}^{(U)}_\text{adv}$ for PGD+SNAP and PGD+Iso[L], where Iso[L] denotes a baseline SNAP alternative employing isotropic Laplace noise augmentation, \ie, without noise shaping. PGD+SNAP achieves better $\mathcal{A}_\text{nat}$ \vs $\mathcal{A}^{(U)}_\text{adv}$ trade-off due to noise shaping..
	%with $\epsilon=(0.031,0.5,12)$, respectively.
	}
	\label{fig::RSComp} 
	\vspace{-0.25cm}
\end{figure}

In order to further quantify importance of \emph{noise shaping}, we also compare PGD+SNAP with PGD+Iso[L], a stronger baseline alternative consisting of \emph{isotropic} Laplace noise augmentation, \ie, \emph{without any noise shaping}. Specifically, in Iso[L], the noise standard deviation is \emph{identical} in each direction, \ie, $\Sigma=\text{Diag}\bigg[\sqrt{\frac{P_\text{noise}}{D}},\dots,\sqrt{\frac{P_\text{noise}}{D}}\bigg]$. 

{Fig.~\ref{fig::RSComp}(b) plots the  $\mathcal{A}_\text{nat}$ \vs  $\mathcal{A}^{(U)}_\text{adv}$ trade-off for PGD+SNAP (\emph{red curve}) and PGD+Iso[L] (\emph{black curve}) by sweeping  $P_\text{noise}$. We find that PGD+SNAP achieves a better $\mathcal{A}_\text{nat}$ \vs  $\mathcal{A}^{(U)}_\text{adv}$ trade-off compared to PGD+Iso[L] by making more efficient use of noise power via noise shaping. Specifically, for $\mathcal{A}^{(U)}_\text{adv}\approx 38$, PGD+SNAP achieves a $\sim 4\%$ higher $\mathcal{A}_\text{nat}$. } 



\begin{table}[t]
	\centering
	\resizebox{0.55\columnwidth}{!}{
	\begin{tabular}{|c|>{\centering\arraybackslash}p{0.9cm}|>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{0.9cm}>{\centering\arraybackslash}p{0.9cm}|>{\centering\arraybackslash}p{0.9cm}| } %
		\hline
		{\makecell{Method}} &  {\makecell{$\mathcal{A}_\text{nat}$} } & {\makecell{$\mathcal{A}^{(\ell_\infty)}_\text{adv}$ \\ {\scriptsize $\epsilon=0.03$} }} & {\makecell{$\mathcal{A}^{(\ell_2)}_\text{adv}$\\ {\scriptsize $\epsilon=0.5$} }} &  {\makecell{$\mathcal{A}^{(\ell_1)}_\text{adv}$\\ {\scriptsize $\epsilon=12$}  }} & {\makecell{$\mathcal{A}^{(U)}_\text{adv}$} } \\ [1.2ex]
		\hline
		{\makecell{PGD}}  & {84.6} & {48.8} & 62.3 & {15.0} & {15.0}   \\
		\hline
		\hline
		\multicolumn{6}{|c|}{\textbf{Noise shaping basis $V=\mathbf{I}_{D\times D}$ }} \\
		\hline
		\hline
		%\cline{1-6}
		 \textbf{+SNAP[G]}  & {80.7}  & \textbf{45.7}  & {66.9}  &  {34.6} &  {31.9} \\
		%\cline{1-6}
		 \textbf{+SNAP[U]}  & \textbf{85.1}  & {42.7}  & \textbf{66.7}  &  {28.6} &  {26.6}  \\
		%\cline{1-6}
		\textbf{+SNAP[L]}  & {83.0}  & {44.8}  & \textbf{68.6}  &  \textbf{40.1} &  \textbf{35.6} \\
    	\hline
		\hline
		\multicolumn{6}{|c|}{\textbf{Noise shaping basis $V=U_{\text{img}}$}} \\
		\hline
		\hline
		%\cline{1-6}
		 \textbf{+SNAP[G]}  & {81.7}  & \textbf{48.9}  & {67.5}  &  \textbf{29.8} &  \textbf{28.7} \\
		%\cline{1-6}
		 \textbf{+SNAP[U]}  & \textbf{82.0}  & {46.6}  & \textbf{67.8}  &  {27.8} &  {25.7}  \\
		%\cline{1-6}
		\textbf{+SNAP[L]}  & {81.7}  & {46.8}  & {65.9}  &  {28.5} &  {27.4} \\

    	\hline %
	\end{tabular}}
	\caption{ResNet-18 CIFAR-10 results showing the impact of noise shaping basis $V$ for $\ell_\infty$-PGD~\citep{madry2018towards} AT framework with SNAP, where SNAP[G], SNAP[U], and SNAP[L] denote shaped noise augmentations with Gaussian, Uniform, and Laplace noise distributions, respectively, and $U_\text{img}$ denotes singular vector basis of the training images.} %
	\label{tab::NoiseBasisComp}
	\vspace{-0.3cm}
\end{table}



\subsection{Role of noise shaping basis $V$}
\label{subsec::NoiseBasis}
 Recall that, for all experiments in the main text, we chose $V=\mathbf{I}_{D\times D}$, \ie, the noise was shaped and added in the standard basis in $\mathbb{R}^D$, where $\mathbf{I}_{D\times D}$ denotes the identity matrix (see equation~1 and Alg.~1 in the main text). 
 %In this section, we explore the impact of noise shaping basis $V$ (see equation~1 and Alg.~1 in the main text).

In this section, we explore the shaped noise augmentation in the \emph{image basis}, \ie, singular vector basis of the training set images. Specifically, we choose $V=U_\text{img}=[\vu_1,\dots,\vu_D]$, where $U_\text{img}$ denotes the singular vector basis of the images in the training set. Thus, the sampled noise vector $\rvn_0$ (see equation~1 in the main text) is scaled by direction-wise standard deviation matrix $\Sigma$ and \emph{rotated} by $U_\text{img}$ before being added to the input image $\vx$. 

The rationale for choosing $V=U_\text{img}$ is as follows: Recent works~\cite{ilyas2019adversarial,shafahi2019adversarial,santurkar2019image} have demonstrated the generative behavior of adversarial perturbations of  networks trained with single-attack AT, \ie, adversarial perturbations of robust networks exhibit semantics similar to the input images. Thus, the perturbation basis (see section~3 in the main text) of the robust networks trained with single-attack AT seems to be aligned with the image basis. 

We repeat the experiments in Table~1 of the main text while keeping all the settings the \emph{same} except for choosing $V=U_\text{img}$ instead of $V=\mathbf{I}_{D\times D}$. Table~\ref{tab::NoiseBasisComp} shows the results. The first three rows correspond to $V=\mathbf{I}_{D\times D}$ and are reproduced from Table~1 of the main text. Note that, in order to preserve $\mathcal{A}_\text{nat}> 81\%$, we need to reduce $P_\text{noise}=60$ when $V=U_\text{img}$.

In Table~\ref{tab::NoiseBasisComp}, we notice that $\mathcal{A}^{(\ell_1)}_{\text{adv}}$ is significantly reduced when $V=U_\text{img}$ as compared to the case $V=\mathbf{I}_{D\times D}$. 
%Specifically, for SNAP[L] and SNAP[G] $\mathcal{A}^{(\ell_1)}_{\text{adv}}$ is 11\% and 5\% lower when $V=U_\text{img}$. 
More interestingly, all three types of noise distributions result in similar values for $\mathcal{A}^{(\ell_1)}_{\text{adv}}$ when $V=U_\text{img}$.
%\ie, when the noise vector is rotated before adding to input. 
%In contrast, we observe large difference in $\mathcal{A}^{(\ell_1)}_{\text{adv}}$ for three noise distributions when $V=\mathbf{I}_{D\times D}$. 
We discuss this phenomenon in the next section,  Sec.~\ref{app::NoiseHist}. 

Table~\ref{tab::NoiseBasisComp} shows that the orientation of a noise vector is as important as its distribution. The simpler choice of $V=\mathbf{I}_{D\times D}$ turns out to be more effective. 

\subsection{Understanding the effectiveness of SNAP[L] for $\ell_\infty$ AT }
\label{app::NoiseHist}
In this subsection, we conduct additional studies to comprehend the following two observations in SNAP: (i) shaped Laplace noise is particularly effective (Table~1 in the main text), and (ii) rotating noise vectors ($V=U_\text{img}$) reduces their effectiveness (Table~\ref{tab::NoiseBasisComp} in this Supplementary). We study the properties of the noise vector $\rvn$ for different noise distributions.

We conjecture that the Laplace distribution is most effective because of its heavier tail compared to Gaussian and Uniform distributions of the same variance. A long-tailed distribution will generate more large magnitude elements in a vector drawn from it and hence is more effective in emulating a strong $\ell_1$-norm bounded perturbation. Furthermore, the standard (un-rotated) basis preserves this unique attribute of samples drawn from such distributions.

This conjecture is validated by Fig.~\ref{fig::NoiseStdHist}(a) which shows that noise samples drawn from the Laplace distribution in the standard basis have the highest average number of dimensions with large ($>0.5$) magnitudes, followed by Gaussian and Uniform distributions. This correlates well with the results in Table~1 in the main text and Table III (first three rows), in that $\mathcal{A}^{(\ell_1)}_\text{adv}$ is the highest for Laplace followed by those for Gaussian and Uniform. Additionally, the use of $V=U_\text{img}$ dissolves this distinction between the three distributions as shown in Fig.~\ref{fig::NoiseStdHist}(b) which explains the similar (and lower)  $\mathcal{A}^{(\ell_1)}_\text{adv}$ values for all three distributions in Table~III.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\linewidth]{figures/NoiseNormHist.pdf}
	\end{center}
	\vspace{-0.4cm}
	\caption{ResNet18 CIFAR-10 results: histograms of the fraction of noise vector dimensions with magnitude (a) $>0.5$ when $V=\mathbf{I}_{D\times D}$, and (b) $>0.4$ when $V=U_{\text{img}}$. Histograms are plotted for 5000 random noise samples $\rvn$. The three shaped noise distributions are from the corresponding networks in Table~\ref{tab::NoiseBasisComp}.}
	\label{fig::NoiseStdHist} 
	\vspace{-0.25cm}
\end{figure}


Thus, we confirm that the type of noise plays an important role in robustifying single-attack $\ell_\infty$ AT frameworks to the union of multiple perturbation models. Specifically, the noise vectors with higher fraction of noise dimensions with larger magnitudes are better at complementing $\ell_\infty$ AT frameworks.

\section{Additional Details}
\label{app::Details}

\subsection{Details of Hyperparameters}

\subsubsection{Attack hyperparameters}

As mentioned in the main text, we follow basic PGD attack formulations of \citet{maini2019adversarial}. We further enhance them to target the full defense -- SN layer -- since SNAPnet is end-to-end differentiable. Specifically, we backpropagate to primary input $\vx$ through the SN layer (see Fig.~4(b) in the main text). Thus, the final shaped noise distribution is exposed to the adversary. We also account for the $\mathbb{E}_\rvn[\cdot]$ (see equation~2 in the main text) by explicitly averaging deep net logits over $N_0$ noise samples \emph{before} computing the gradient, which eliminates any gradient obfuscation, and was shown to be the strongest attack against noise augmented models~\cite{salman2019provably}. We choose $N_0=8$ for all our attack evaluations. 

For $\ell_2$ and $\ell_\infty$ PGD attacks, we choose steps size $\alpha=0.1\epsilon$. For $\ell_1$ PGD attacks, we choose the exact same configuration as \citet{maini2019adversarial}. 

\subsubsection{Training hyperparameters}

As mentioned in the main text, we introduce SNAP without changing any hyperparameters of BASE() AT. All BASE() and BASE()+SNAP  training runs on CIFAR-10 employ SGD optimizer with a fixed momentum of $0.9$, batch size of $250$, and weight decay of $2\times 10^{-4}$. Also, while accounting for the $\mathbb{E}_\rvn[\cdot]$ (see equation~2 in the main text), note that $N_0=1$ suffices during BASE()+SNAP training. Below we provide specific details for each SOTA AT framework:

{\textbf{BASE() $\equiv$ PGD~\cite{madry2018towards} on CIFAR-10:}}

$\ell_\infty$-PGD AT employed $\ell_\infty$-bounded PGD-$K$ attack with  $\epsilon=0.031$, step size $\alpha=0.008$, and $K=10$. For $\ell_2$-PGD AT, we used $\ell_2$-bounded PGD-$K$ attack with $\epsilon=0.5$, step size $\alpha=0.125$ and $K=10$. 
Following \citet{rice2020overfitting}, we employed $100$ epochs for PGD AT with step learning rate (LR) schedule, where LR was decayed from 0.1 to 0.01 at epoch 96. Following \citet{maini2019adversarial}, we also employed \emph{their} cyclic LR schedule to achieve superconvergence in 50 epochs. Following \citet{maini2019adversarial}, we set weight decay to $5\times 10^{-4}$ in PGD AT. 

In PGD+SNAP, the noise variances were updated every $U_f=10$ epochs and we use $P_\text{noise}=160$ in Tables~1,2, and 3 in the main text. 



{\textbf{BASE() $\equiv$ TRADES~\cite{zhang2019theoretically} on CIFAR-10:}}

Following \citet{zhang2019theoretically}, TRADES AT employed $\ell_\infty$-bounded perturbations with $\epsilon=0.031$, step size $\alpha=0.007$, and attack steps $K=10$. We set TRADES parameter $1/\lambda=5$, which controls the weighing of its robustness regularizer. It was trained for 100 epochs with step LR schedule, where LR was decayed to \{0.01,0.001,0.0001\} at the epochs $\{75,90,100\}$, respectively. Following \citet{maini2019adversarial}, we also employed \emph{their} cyclic LR schedule to achieve superconvergence in 50 epochs, while keeping all other settings same. 

In TRADES+SNAP, the noise variances were updated every $U_f=10$ epochs and we use $P_\text{noise}=120$ in Tables~2 and 3 in the main text. 

{\textbf{BASE() $\equiv$ FreeAdv~\cite{shafahi2019adversarial} on CIFAR-10:}}

Following \citet{shafahi2019adversarial}, FreeAdv AT was trained for 25 epochs, each consisting of a replay of 8. It employed $\ell_\infty$ perturbations with $\epsilon=0.031$. The learning rate was decayed to $\{0.01,0.001,0.0001\}$ at the epochs $\{13,19,23\}$, respectively. 

In FreeAdv+SNAP, the noise variances were updated every $U_f=5$ epochs, since the replay of 8 scales down the total number of epochs. Also, we use $P_\text{noise}=160$ in Tables~2 and 3 in the main text. 


{\textbf{BASE() $\equiv$ FastAdv~\cite{wong2020fast} on CIFAR-10:}}

Following \citet{wong2020fast}, FastAdv AT employed single-step $\ell_\infty$ norm bounded FGSM  attack with $\epsilon=8/255$, step size $\alpha=10/255$, and random noise initialization. It was trained for 50 epochs with the \emph{same} cyclic LR schedule used by \citet{wong2020fast}. We used weight decay of $5\times 10^{-4}$.

In FastAdv+SNAP, the noise variances were updated every $U_f=10$ epochs and we use $P_\text{noise}=200$ in Tables~2 and 3 in the main text. 
 
{\textbf{BASE() $\equiv$ FreeAdv~\cite{shafahi2019adversarial} on ImageNet:}}

Following \citet{shafahi2019adversarial}, FreeAdv AT was trained for 25 epochs, each consisting of a replay of 4. It employed $\ell_\infty$ perturbations with $\epsilon=4/255$, \emph{identical} to the authors' original setup. The LR was decayed by 0.1 every 8 epochs, starting with the initial LR of 0.1. We used weight decay of $1\times 10^{-4}$.

In FreeAdv+SNAP, the noise variances were updated every $U_f=5$ epochs, since the replay of 4 scales down the total number of epochs. Also, we use $P_\text{noise}=4500$ in Table~4 in the main text, which corresponds to noise standard deviation of $\sim 0.17$ per pixel \emph{on average}. 

{\textbf{MSD-$K$~\cite{maini2019adversarial} experiments for $K\in\{ 30, 20, 10, 5 \}$:}}

\citet{maini2019adversarial} report results for only MSD-50 in their paper. We produce MSD-$K$ results using their publicly available code. While reducing the number of steps in MSD, we \emph{appropriately} increase the step size $\alpha$ for the attack. For MSD-50, \citet{maini2019adversarial} used $\alpha=(0.003,0.05,0.05)$ for $(\ell_\infty, \ell_2, \ell_1)$ perturbation models, respectively. We proportionately increase step size to $\alpha=(0.005,0.084,0.084)$ and $\alpha=(0.0075,0.125,0.125)$ for MSD-30 and MSD-20, respectively. 

For MSD-10 and MSD-5, we choose $\alpha=(0.0075,0.125,0.125)$, since we found that further increasing step size $\alpha$ for them leads to \emph{lower} final adversarial accuracy. 

Other than the step-size, we do \emph{not} make any change to the original code by \citet{maini2019adversarial}. 

\subsection{Details about SNAP}

\subsubsection{Distribution Update Epoch}

In SNAP distribution update epoch (see Algorithm~1 in the main text), we employ $\ell_2$ norm-bounded PGD attack to compute perturbation vectors $\bm{\eta}$. We use only  20\% of the training data, which is randomly selected during every SNAP update epoch. Recall that normalized root mean squared projections of $\bm{\eta}$ dictate the updated noise variances (equation~3 in the main text). Here are more details specific to CIFAR-10 and ImageNet datasets:

CIFAR-10: we employ 10 step $\ell_2$-PGD attack with $\epsilon=1.8$ and $N_0=4$. 

ImageNet: we employ 4 step $\ell_2$-PGD attack with $\epsilon=4.0$ and $N_0=1$.

Note that $\ell_2$ norm bound $\epsilon$ for the PGD attack here does not play any role, since $\bm{\eta}$ perturbation projections anyway get normalized. 


\subsubsection{Noise variance initialization in SNAP}

In SNAP, we initialize the noise variances to be uniform across all dimensions. Specifically, in Algorithm~1 in the main text, $\Sigma_0=\text{Diag}\bigg[\sqrt{\frac{P_\text{noise}}{D}},\dots,\sqrt{\frac{P_\text{noise}}{D}}\bigg]$ for a given value of $P_\text{noise}$. 

\section{Accompanying Code and Pretrained Models}

As a part of this supplementary material, we share our code to reproduce PGD+SNAP and TRADES+SNAP results on CIFAR-10 (Table~2 in the main text) and FreeAdv+SNAP results on ImageNet (Table~4 in the main text). We also share corresponding pretrained models to facilitate quick reproduction of our results. Code and models are available at link the \href{https://github.com/adpatil2/SNAP}{https://github.com/adpatil2/SNAP}.

% \subsection{Code and models are available at link: \url{https://github.com/adpatil2/SNAP}}


\end{appendices}
% \end{document}
